Error-Tolerant Quantum State Discrimination: Optimization and Quantum Circuit Synthesis

We develop error-tolerant quantum state discrimination(QSD) strategies that maintain reliable performance under moderate noise. Two complementary approaches are proposed: CrossQSD, which generalizes unambiguous discrimination with tunable confidence bounds to balance accuracy and efficiency, and FitQSD, which optimizes the measurement outcome distribution to approximate that of the ideal noiseless case. Furthermore, we provide a unified hybrid-objective QSD framework that continuously interpolates between minimum-error discrimination (MED) and FitQSD, allowing flexible trade-offs among competing objectives. The associated optimization problems are formulated as convex programs and efficiently solved via disciplined convex programming or, in many cases, semidefinite programming. Additionally, a circuit synthesis framework based on a modified Naimark dilation and isometry synthesis enables hardware-efficient implementations with substantially reduced qubit and gate resources. An open-source toolkit automates the full optimization and synthesis workflow, providing a practical route to QSD on current quantum devices.

==> figures/fitqsd_table.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance of FitQSD using MOSEK solver at precisions $\epsilon = 10^{-8}, 10^{-9}$. %Shows $L_2$ norm and $\psucc$ for MinL1, MinSS, MECO methods across $\lSDP$.
    }
    \label{tab:fitqsd_results}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c |c |c |c |c |c |c}
        \hline
        \multirow{2}{*}{\textbf{$\lSDP$}} & \multicolumn{2}{c|}{\textbf{MinL1}} & \multicolumn{2}{c|}{\textbf{MinSS}} & \multicolumn{2}{c}{\textbf{MECO}}                                                                                         \\
        \cline{2-7}
                                        & \textbf{$L_2$},\, ($\epsilon$)        & \textbf{$\psucc$}         & \textbf{$L_2$},\, ($\epsilon$)       & \textbf{$\psucc$} & \textbf{$L_2$},\, ($\epsilon$) & \textbf{$\psucc$} \\
        \hline
        \multirow{2}{*}{$1.00 \times 10^{-6}$}           & 2.62e-7 (1e-8)                     & 0.81089                            & 4.26e-5 (1e-8)                    & 0.81086                    & 3.06e-7 (1e-8)              & 0.81089                    \\
                                        & 2.48e-7 (1e-9)                     & 0.81089                            & 2.04e-5 (1e-9)                    & 0.81088                    & 3.03e-7 (1e-9)              & 0.81089                    \\
        \hline
        \multirow{2}{*}{$1.00 \times 10^{-5}$}           & 2.49e-6 (1e-8)                     & 0.81089                            & 4.40e-5 (1e-8)                    & 0.81086                    & 3.05e-6 (1e-8)              & 0.81089                    \\
                                        & 2.48e-6 (1e-9)                     & 0.81089                            & 2.29e-5 (1e-9)                    & 0.81087                    & 3.03e-6 (1e-9)              & 0.81089                    \\
        \hline
        \multirow{2}{*}{$1.00 \times 10^{-4}$}           & 2.50e-5 (1e-8)                     & 0.81087                            & 5.94e-5 (1e-8)                    & 0.81084                    & 3.03e-5 (1e-8)              & 0.81085                    \\
                                        & 2.79e-5 (1e-9)                     & 0.81086                            & 3.58e-5 (1e-9)                    & 0.81086                    & 3.03e-5 (1e-9)              & 0.81085                    \\
        \hline
        \multirow{2}{*}{$1.00 \times 10^{-3}$}           & 2.97e-4 (1e-8)                     & 0.81048                            & 2.75e-4 (1e-8)                    & 0.81065                    & 3.03e-4 (1e-8)              & 0.81047                    \\
                                        & 3.03e-4 (1e-9)                     & 0.81047                            & 3.16e-4 (1e-9)                    & 0.81062                    & 3.03e-4 (1e-9)              & 0.81047                    \\
        \hline
        \multirow{2}{*}{$1.00 \times 10^{-2}$}           & 3.04e-3 (1e-8)                     & 0.80661                            & 2.50e-3 (1e-8)                    & 0.80871                    & 3.04e-3 (1e-8)              & 0.80661                    \\
                                        & 3.04e-3 (1e-9)                     & 0.80661                            & 2.50e-3 (1e-9)                    & 0.80871                    & 3.04e-3 (1e-9)              & 0.80661                    \\
        \hline
        \multirow{2}{*}{$1.00 \times 10^{-1}$}           & 3.19e-2 (1e-8)                     & 0.76599                            & 2.83e-2 (1e-8)                    & 0.78046                    & 3.19e-2 (1e-8)              & 0.76599                    \\
                                        & 3.19e-2 (1e-9)                     & 0.76599                            & 2.83e-2 (1e-9)                    & 0.78046                    & 3.19e-2 (1e-9)              & 0.76599                    \\
        \hline
    \end{tabular}
\end{table}

==> figures/sticky_notes.tex <==
\usetikzlibrary{shapes.geometric, arrows, shadows}

\tikzset{
    sticky note/.style={
        rectangle,
        rounded corners=5pt,
        minimum height=2cm,
        minimum width=5cm,
        fill=yellow!20,
        draw=yellow!50!black,
        thick,
        drop shadow={shadow xshift=3pt, shadow yshift=-3pt},
        % rotate=-2, % Slight tilt for sticky note effect
        align=center,
        font=\normalsize,
    }
}

\begin{tikzpicture}
    \node[sticky note] at (0,0) {
        \begin{minipage}{4.5cm}
            \begin{align*}
                \ket{\psi_{1}} = \ket{0}                           \\
                \ket{\psi_{2}} = \dfrac{\ket{0}+\ket{1}}{\sqrt{2}} \\
                S_{prior} = \{p_{1}, p_{2}\} = \{0.5, 0.5\}
            \end{align*}
        \end{minipage}
    };
\end{tikzpicture}

==> figures/test_forest.tex <==
% \documentclass[border=20pt,tikz]{standalone}

\usepackage[edges]{forest}

\forestset{
  direction switch/.style={
    for tree={edge+=thick, font=\sffamily},
    where level>=1{folder, grow'=0}{for children=forked edge},
    where level=3{}{draw},
  },
}
% \begin{document}

\begin{forest}
  % forest preamble: determine layout and format of tree
  direction switch
  [Redmine Project Organization
    [Blockchain
      [HashGraph
      ]
      [Vue-Dapp
        [Docsaurus]
        [Deploy to MainNet]
        [Update Todolist]
      ]
      [IPFS Dapp
      	[Drizzle Truffle]
      	[Solidity Contract]
      	[Deploy to Surge]
      ]
    ]
    [Academic
      [ENGR Year 4
      	[CENG 4B]
      	[CENG 4A]
      ]
      [Tutorials
        [Voting Dapp]
      ]
      [Article Summary
      	[Vyper + Truffle]
      	[Tensorflow]
      	[HashGraph]
      ]
    ]
    [Job Hunt
      [First Job
        [Blockchain]
        [AI]
      ]
      [Scripts
      	[Go-api]
      	[Indeed Scrapper]
      	[Uvic Scrapper]
      ]
    ]
    [AI
    	[Chatbots]
    	[Tensorflow]
    ]
    [Projects
    	[Portfolio Website]
    	[Notes --- Vuepress]
    ]
  ]
\end{forest}
% \end{document}
